Seven years of Tunka-Rex operation

The Tunka Radio Extension (Tunka-Rex) is a digital antenna array located in the Tunka Valley in Siberia, which measures the radio emission of cosmic-ray air-showers with energies up to EeV. Tunka-Rex is externally triggered by the Tunka-133 air-Cherenkov timing array (during nights) and by the Tunka-Grande array of particle detectors (remaining time). These three arrays comprise the cosmic-ray extension of the Tunka Advanced Instrument for cosmic rays and Gamma Astronomy (TAIGA). The configuration and analysis pipeline of Tunka-Rex have significantly changed over its runtime. Density of the antennas was tripled and the pipeline has become more developed forming now sophisticated piece of reconstruction software. During its lifecycle Tunka-Rex has demonstrated that a cost-effective and full duty-cycle radio detector can reconstruct the energy and shower maximum with a precision comparable to optical detectors. Moreover, it was shown that cosmic-ray instruments, that use different detection techniques and are placed in different locations, can be cross-calibrated via their radio extensions. These results show the prospects of application of the radio technique for future large-scale experiments for cosmic-ray and neutrino detection. For the time being Tunka-Rex has ceased active measurements and focuses on the data analysis and publication of corresponding software and data in an open-access data center with online analysis features. In this report we present the current status of the array and give an overview of the results achieved during these years as well as discuss upcoming improvements in instrumentation and data analysis, which can be applied for the future radio arrays.

==> Makefile <==
FILE = kostunin-icrc2019

PDFLATEX = pdflatex
BIBTEX = bibtex

PDF = ${FILE}.pdf

all :	
	${PDFLATEX} ${FILE}.tex
	${BIBTEX} ${FILE}
	${PDFLATEX} ${FILE}.tex
	${PDFLATEX} ${FILE}.tex
	${PDFLATEX} collaboration.tex

# Various cleaning options
clean :
	/bin/rm -f  *.log *.aux *.dvi *.bbl *.blg *.bm *.toc *.out \
	*Notes.bib *.ps

